Modelling of an Ionic Electroactive Polymer by the Thermodynamics of Linear Irreversible Processes

Ionic polymer-metal composites consist in a thin film of electro-active polymers (Nafion R for example) sandwiched between two metallic electrodes. They can be used as sensors or actuators. The polymer is saturated with water, which causes a complete dissociation and the release of small cations. The strip undergoes large bending motions when it is submitted to an orthogonal electric field and vice versa. We used a continuous medium approach and a coarse grain model; the system is depicted as a deformable porous medium in which flows an ionic solution. We write microscale balance laws and thermodynamic relations for each phase, then for the complete material using an average technique. Entropy production, then constitutive equations are deduced : a Kelvin-Voigt stress-strain relation, generalized Fourier's and Darcy's laws and a Nernst-Planck equation. We applied this model to a cantilever E.A.P. strip undergoing a continuous potential difference (static case); a shear force may be applied to the free end to prevent its displacement. Applied forces and deflection are calculated using a beam model in large displacements. The results obtained are in good agreement with the experimental data published in the literature.

==> referenc.tex <==
%%%%%%%%%%%%%%%%%%%%%%%% referenc.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample references
% %
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer-Verlag %%%%%%%%%%%%%%%%%%%%%%%%%%
%
% BibTeX users please use
% \bibliographystyle{}
% \bibliography{}
%

\begin{thebibliography}{99.}

\bibliographystyle{plain}
\bibliography{D:/Recherche/Articles/biblio.bib}
%\graphicspath{{D:/Enseignements/Meca-flu-L2_ME403/TD/Figures-TD/}}
%\bibliography{$HOME/quelque/part/exemple.bib}

\end{thebibliography}

